Towards Optimization and Model Selection for Domain Generalization: A Mixup-guided Solution

The distribution shifts between training and test data typically undermine the performance of models. In recent years, lots of work pays attention to domain generalization (DG) where distribution shifts exist, and target data are unseen. Despite the progress in algorithm design, two foundational factors have long been ignored: 1) the optimization for regularization-based objectives, and 2) the model selection for DG since no knowledge about the target domain can be utilized. In this paper, we propose Mixup guided optimization and selection techniques for DG. For optimization, we utilize an adapted Mixup to generate an out-of-distribution dataset that can guide the preference direction and optimize with Pareto optimization. For model selection, we generate a validation dataset with a closer distance to the target distribution, and thereby it can better represent the target data. We also present some theoretical insights behind our proposals. Comprehensive experiments demonstrate that our model optimization and selection techniques can largely improve the performance of existing domain generalization algorithms and even achieve new state-of-the-art results.

==> tab/dsads.tex <==
\begin{table}[t!]
\centering
\caption{Results on DSADS. The \textbf{bold} items are the best results.}
\label{tab-dsads-r}
\begin{tabular}{lccccc}
\toprule
          & 0              & 1              & 2              & 3              & AVG            \\
          \midrule
ERM       & 89.69          & 81.45          & 81.05          & 78.20          & 82.60          \\
DANN      & 87.54          & 81.27          & 78.42          & 83.03 & 82.57          \\
ANDMask   & 85.35          & 73.07          & 85.04          & 82.06          & 81.38          \\
GILE      & 79.67          & 75.00          & 77.00          & 67.00          & 74.65          \\
DANN+Ours & \textbf{93.33}& 	\textbf{88.77}& 	\textbf{91.75}& 	\textbf{84.78}& 	\textbf{89.66} 
\\ \bottomrule
\end{tabular}
\end{table}

==> tab/pamap.tex <==
\begin{table}[t!]
\centering
\caption{Results on PAMAP2. The \textbf{bold} items are the best results.}
\label{tab-pamap-r}
\begin{tabular}{lccccc}
\toprule
          & 0              & 1             & 2              & 3              & AVG           \\ \midrule
ERM       & 87.28          & 73.1          & 49.03          & 78.76          & 72.04         \\
DANN      & 88.93 & 75.6          & 47.35          & 86.78          & 74.66         \\
ANDMask   & 88.22          & 79.11         & 53.35          & 83.22          & 75.97         \\
GILE      & 83.33          & 68.67         & 44.00          & 76.67          & 68.25         \\
DANN+Ours & \textbf{89.23}& 	\textbf{81.36}& 	\textbf{61.71}& 	\textbf{89.28}& 	\textbf{80.40} 
\\ \bottomrule
\end{tabular}
\end{table}

==> tab/usc.tex <==
\begin{table}[t!]
\centering
\caption{Results on USC-HAD. The \textbf{bold} items are the best results.}
\label{tab-usc-r}
\begin{tabular}{lccccc}
\toprule
          & 0              & 1              & 2              & 3             & AVG            \\ \midrule
ERM       & 80.33          & 59.88          & 74.15          & 73.93         & 72.07          \\
DANN      & 81.33 & 64.02 & 72.91          & 66.37         & 71.16          \\
ANDMask   & 79.51          & 61.53          & 76.32          & 65.52         & 70.72          \\
GILE      & 78.67          & 63.00          & \textbf{77.00} & 61.67         & 70.08          \\
DANN+Ours & \textbf{81.98}& 	\textbf{64.32}& 	74.84& 	\textbf{78.40}& 	\textbf{74.89} 
\\ \bottomrule
\end{tabular}
\end{table}
